Investigating Non-local Features for Neural Constituency Parsing

Thanks to the strong representation power of neural encoders, neural chart-based parsers have achieved highly competitive performance by using local features. Recently, it has been shown that non-local features in CRF structures lead to improvements. In this paper, we investigate injecting non-local features into the training process of a local span-based parser, by predicting constituent n-gram non-local patterns and ensuring consistency between non-local patterns and local constituents. Results show that our simple method gives better results than the self-attentive parser on both PTB and CTB. Besides, our method achieves state-of-the-art BERT-based performance on PTB (95.92 F1) and strong performance on CTB (92.31 F1). Our parser also achieves better or competitive performance in multilingual and zero-shot cross-domain settings compared with the baseline.

==> tex_files/experiment_table.tex <==
\begin{table}[]
    \fontsize{10}{12}\selectfont
    \centering
    \begin{tabular}{lccc}
        % \hline
        % \multicolumn{4}{c}{PTB} \\
        \hline
        Model & LR & LP & F1 \\
        \hline
        \citet{liu-zhang-2017-order} $\diamond$ & - & - & 95.71 \\
        \citet{san-constituency} & 95.46 & 95.73 & 95.59 \\
        \citet{head-driven} & 95.51 & 95.93 & 95.72 \\
        \citet{head-driven} * & 95.70 & 95.98 & 95.84 \\
        \citet{constituency-crf} & 95.53 & 95.85 & 95.69 \\
        \citet{constituency-point} & - & - & 95.48 \\
        % \citet{incremental-parsing} & 95.55 & 96.04 & 95.79 \\
        \citet{span-attention} & 95.58 & 96.11 & 95.85 \\
        \hline
        \multicolumn{4}{c}{This work} \\
        \hline
        \citet{san-constituency} $\dagger$ & 95.56 & 95.89 & 95.72 \\
        % \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{95.49} & \multirow{2}{*}{96.07} & \multirow{2}{*}{95.78} \\
        %  + pattern loss & & & \\
        % %  \hdashline
        %  \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{95.70} & \multirow{2}{*}{96.14} & \multirow{2}{*}{95.92} \\
        %  + pattern\&constraint losses &  &  &  \\
        NFC w/o $\mathcal{L}_{reg}$ & 95.49 & 96.07 & 95.78 \\
        % Ours & {\bf 95.70} & {\bf 96.14} & {\bf 95.92} \\
        NFC & {\bf 95.70} & {\bf 96.14} & {\bf 95.92} \\
        \hline
    \end{tabular}
    \caption{Constituency parsing performance (w/ BERT) on the test set of PTB. $\dagger$ indicates our reproduced results, which is also the baseline that our method is built upon. * indicates training with extra supervision from dependency parsing data. $\diamond$ indicates that the results are reported by the re-implementation of \citet{cross-domain-parser}. }
    \label{tab:ptb}
\end{table}


\begin{table}[t!]
    \fontsize{10}{12}\selectfont
    \centering
    \begin{tabular}{lccc}
    \hline
        Model & LR & LP & F1 \\
        \hline
        % \multicolumn{4}{c}{w/ BERT} \\
        % \hline
        \citet{liu-zhang-2017-order} $\diamond$ & - & - & 91.81 \\
        \citet{san-constituency} & 91.55 & 91.96 & 91.75 \\
        \citet{head-driven} * & 92.03 & 92.33 & 92.18 \\
        \citet{constituency-crf} & 92.04 & 92.51 & 92.27 \\
        % \citet{incremental-parsing} & 93.40 & 93.80 & 93.59 \\
        \citet{span-attention} & 92.14 & 92.25 & 92.20 \\
        % \citet{label-attention-parsing}* & 91.85 & {\bf 93.45} & {\bf 92.64} \\
        \hline
        \multicolumn{4}{c}{This work} \\
        \hline
        \citet{san-constituency} $\dagger$ & 91.80 & 92.23 & 91.98 \\
        % \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{91.87} & \multirow{2}{*}{92.40} & \multirow{2}{*}{92.13} \\
        %  + pattern loss & & & \\
        % %  \hdashline
        %  \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{92.17} & \multirow{2}{*}{92.63} & \multirow{2}{*}{92.31} \\
        %  + pattern\&constraint losses &  &  &  \\
        NFC w/o $\mathcal{L}_{reg}$ & 91.87 & 92.40 & 92.13 \\
        % Ours & {\bf 92.17} & {\bf 92.45} & {\bf 92.31} \\
        NFC & {\bf 92.17} & {\bf 92.45} & {\bf 92.31} \\
        \hline
    \end{tabular}
    \caption{Constituency parsing performance (w/ BERT) on the test set of CTB 5.1. The symbols ($\dagger$, * and $\diamond$) are explained in Table~\ref{tab:ptb}.}
    \label{tab:ctb}
\end{table}


% \begin{table}[]
%     \fontsize{10}{12}\selectfont
%     \centering
    
%     \begin{tabular}{lccc}
%     \hline
%         Model & LR & LP & F1 \\
%         \hline
%         % \multicolumn{4}{c}{w/ BERT} \\
%         % \hline
%         \citet{liu-zhang-2017-order} $\diamond$ & - & - & 95.71 \\
%         \citet{san-constituency} & 95.46 & 95.73 & 95.59 \\
%         \citet{head-driven} & 95.51 & 95.93 & 95.72 \\
%         \citet{head-driven} * & 95.70 & 95.98 & 95.84 \\
%         \citet{constituency-crf} & 95.53 & 95.85 & 95.69 \\
%         \citet{constituency-point} & - & - & 95.48 \\
%         \citet{incremental-parsing} & 95.55 & 96.04 & 95.79 \\
%         \citet{span-attention} & 95.58 & 96.11 & 95.85 \\
%         \hline
%         \multicolumn{4}{c}{This work} \\
%         \hline
%         \citet{san-constituency} $\dagger$ & 95.56 & 95.89 & 95.72 \\
%         % \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{95.49} & \multirow{2}{*}{96.07} & \multirow{2}{*}{95.78} \\
%         %  + pattern loss & & & \\
%         % %  \hdashline
%         %  \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{95.70} & \multirow{2}{*}{96.14} & \multirow{2}{*}{95.92} \\
%         %  + pattern\&constraint losses &  &  &  \\
%         Ours w/o $\mathcal{L}_{reg}$ & 95.49 & 96.07 & 95.78 \\
%         % Ours & {\bf 95.70} & {\bf 96.14} & {\bf 95.92} \\
%         Ours & {\bf 95.70} & {\bf 96.14} & {\bf 95.92} \\
%         \hline
%     \end{tabular}
%      \subcaption{Constituency parsing performance (w/ BERT) on the test set of PTB. }
%     \bigskip
%     \begin{tabular}{lccc}
%     \hline
%         Model & LR & LP & F1 \\
%         \hline
%         % \multicolumn{4}{c}{w/ BERT} \\
%         % \hline
%         \citet{liu-zhang-2017-order} $\diamond$ & - & - & 91.81 \\
%         \citet{san-constituency} & 91.55 & 91.96 & 91.75 \\
%         \citet{head-driven} * & 92.03 & 92.33 & 92.18 \\
%         \citet{constituency-crf} & 92.04 & 92.51 & 92.27 \\
%         % \citet{incremental-parsing} & 93.40 & 93.80 & 93.59 \\
%         \citet{span-attention} & 92.14 & 92.25 & 92.20 \\
%         \citet{label-attention-parsing}* & 91.85 & {\bf 93.45} & {\bf 92.64} \\
%         \hline
%         \multicolumn{4}{c}{This work} \\
%         \hline
%         \citet{san-constituency} $\dagger$ & 91.80 & 92.23 & 91.98 \\
%         % \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{91.87} & \multirow{2}{*}{92.40} & \multirow{2}{*}{92.13} \\
%         %  + pattern loss & & & \\
%         % %  \hdashline
%         %  \citet{kitaev-etal-2019-multilingual} $\dagger$ & \multirow{2}{*}{92.17} & \multirow{2}{*}{92.63} & \multirow{2}{*}{92.31} \\
%         %  + pattern\&constraint losses &  &  &  \\
%         Ours w/o $\mathcal{L}_{reg}$ & 91.87 & 92.40 & 92.13 \\
%         % Ours & {\bf 92.17} & {\bf 92.63} & {\bf 92.31} \\
%         Ours & {\bf 92.17} & 92.63 & 92.31 \\
%         \hline
%     \end{tabular}
%     \subcaption{Constituency parsing performance (w/ BERT) on the test set of CTB 5.1. }
    
%     \caption{ $\dagger$ indicates our reproduced results, which is also the baseline that our method is built upon. Star (*) indicates training with extra supervision from dependency parsing data. $\diamond$ indicates that the results are reported by the re-implementation of \citet{cross-domain-parser}. }
%     \label{tab:ptb}
% \end{table}
